Concave Utility Reinforcement Learning with Zero-Constraint Violations

We consider the problem of tabular infinite horizon concave utility reinforcement learning (CURL) with convex constraints. For this, we propose a model-based learning algorithm that also achieves zero constraint violations. Assuming that the concave objective and the convex constraints have a solution interior to the set of feasible occupation measures, we solve a tighter optimization problem to ensure that the constraints are never violated despite the imprecise model knowledge and model stochasticity. We use Bellman error-based analysis for tabular infinite-horizon setups which allows analyzing stochastic policies. Combining the Bellman error-based analysis and tighter optimization equation, for $T$ interactions with the environment, we obtain a high-probability regret guarantee for objective which grows as $\Tilde{O}(1/\sqrt{T})$, excluding other factors. The proposed method can be applied for optimistic algorithms to obtain high-probability regret bounds and also be used for posterior sampling algorithms to obtain a loose Bayesian regret bounds but with significant improvement in computational complexity.

==> abstract.tex <==
\begin{abstract}
We consider the problem of tabular infinite horizon concave utility reinforcement learning (CURL) with convex constraints.
For this, we propose a model-based learning algorithm that achieves zero constraint violations. Assuming that the concave objective and the convex constraints have a solution interior to the set of feasible occupation measures, we solve a tighter optimization problem to ensure that the constraints are never violated despite the imprecise model knowledge and model stochasticity. We use Bellman error-based analysis for tabular infinite-horizon setups which allows analyzing stochastic policies. 
Combining the Bellman error-based analysis and tighter optimization equation, for $T$ interactions with the environment, we obtain a regret guarantee for objective which grows as $\Tilde{O}(1/\sqrt{T})$, excluding other factors.
\end{abstract}

==> algorithm.tex <==
\section{Algorithm}
\noindent We now present our algorithm \NAM\ and the key ideas used in designing the algorithm. Note that if the agent is aware of the true transition $P$, it can solve the following optimization problem for the optimal feasible policy.
\begin{align}
        \max_{\rho(s,a)} f\big(\sum\nolimits_{s,a}r(s, a)\rho(s,a)\big) \label{eq:optimization_equation}
\end{align}
with the following set of constraints,
\begin{align}
    &\sum\nolimits_{s,a} \rho(s, a) = 1,\ \  \rho(s, a) \geq 0 \label{eq:valid_prob_constrant}\\
    &\sum\nolimits_{a\in\mathcal{A}}\rho(s',a) = \sum\nolimits_{s,a}P(s'|s, a)\rho(s, a)\label{eq:transition_constraint}\\
    &g\big(\sum\nolimits_{s,a}c_1(s, a)\rho(s,a), \cdots, \sum\nolimits_{s,a}c_d(s, a)\rho(s,a)\big) \leq 0\label{eq:cmdp_constraints}
\end{align}
for all $ s'\in\mathcal{S},~\forall~s\in\mathcal{S},$ and $\forall~a\in\mathcal{A}$.
Equation \eqref{eq:transition_constraint} denotes the constraint on the transition structure for the underlying Markov Process. Equation \eqref{eq:valid_prob_constrant} ensures that the solution is a valid probability distribution. Finally, Equation \eqref{eq:cmdp_constraints} are the constraints for the constrained MDP setup which the policy must satisfy. Using the solution for $\rho$, we can obtain the optimal policy as:
\begin{align}
    \pi^*(a|s) = \frac{\rho(s,a)}{\sum_{b\in\mathcal{A}}\rho(s,b)} \forall\ s,a
\end{align}
However, the agent does not have the knowledge of $P$ to solve this optimization problem, and thus starts learning the transitions with an arbitrary policy. We first note that if the agent does not have complete knowledge of the transition $P$ of the true MDP $\mathcal{M}$, it should be conservative in its policy to allow room to violate constraints. Based on this idea, we formulate the $\epsilon$-tight optimization problem by modifying the constraint in Equation \eqref{eq:cmdp_constraints} as.
\begin{align}
     g\big(\sum\nolimits_{s,a}(c_1\rho_\epsilon)(s,a), \cdots, \sum\nolimits_{s,a}(c_1\rho_\epsilon)(s,a)\big) \leq -\epsilon \label{eq:eps_cmdp_constraints}
\end{align}
Let $\rho_\epsilon$ be the solution of the $\epsilon$-tight optimization problem, then the optimal conservative policy becomes:
\begin{align}
    \pi_\epsilon^*(a|s) = \frac{\rho_\epsilon(s,a)}{\sum\nolimits_{b\in\mathcal{A}}\rho_\epsilon(s,b)} \forall\ s,a
\end{align}
We are now ready to design our algorithm \NAM\ which is based on the optimism principle  \citep{jaksch2010near}. The \NAM\ algorithm is presented in Algorithm \ref{alg:algorithm}. The algorithm proceeds in epochs $e$. The algorithm maintains three key variables $\nu_e(s,a)$, $N_e(s,a)$, and $\hat{P}(s,a,s')$ for all $s,a$. $\nu_e(s,a)$ stores the number of times state-action pair $(s,a)$ are visited in epoch $e$. $N_e(s,a)$ stores the number of times $(s,a)$ are visited till the start of epoch $e$.
$\hat{P}(s,a,s')$ stores the number of times the system transitions to state $s'$ after taking action $a$ in state $s$. Another key parameter of the algorithm is $\epsilon_e = K\sqrt{(\log t_e)/t_e}$ where $t_e$ is the start time of the epoch $e$ and $K$ is a configurable constant. Using these variables, the agent solves for the optimal $\epsilon_e$-conservative policy for the optimistic MDP by replacing the constraints in Equation \eqref{eq:transition_constraint} by:
\begin{align}
    &\sum\nolimits_{a\in\mathcal{A}}\rho(s',a) \le \sum\nolimits_{s,a}\Tilde{P}_e(s'|s, a)\rho(s, a)\label{eq:opt_eps_transition_constraint}\\
    & \Tilde{P}_e(s'|s, a) > 0, \sum\nolimits_{s'}\Tilde{P}_e(s'|s, a)=1\label{eq:boundary}\\
    &\|\Tilde{P}_e(\cdot|s,a) - \frac{\hat{P}(s,a,\cdot)}{1\vee N_e(s,a)}\|_1 \le \sqrt{\frac{14S\log(2At)}{1\vee N_e(s,a)}}\label{eq:opt_transition_probability}  
\end{align}
for all $ s'\in\mathcal{S},\forall s\in\mathcal{S},$ and $\forall a\in\mathcal{A}$ and $x \vee y = \max(x,y)$. Equation \eqref{eq:opt_transition_probability} ensures that the agent searches for optimistic policy in the confidence intervals of the transition probability estimates. 

Combining the right hand side of \eqref{eq:opt_eps_transition_constraint} with \eqref{eq:valid_prob_constrant} gives
\begin{align}
\sum\nolimits_{s'} \sum\nolimits_{s,a}\Tilde{P}_e(s'|s, a)\rho(s, a) = 1 \nonumber =  \sum\nolimits_{s',a} \rho(s', a) 
\end{align}
Thus, joint with \eqref{eq:opt_eps_transition_constraint}, we see that equality in \eqref{eq:opt_eps_transition_constraint} will be satisfied at the boundary as $\sum_{a}\rho(s',a)$ for some $s'$ can never exceed the boundary to compensate for another $s'$ and hence, for all $s'$, $\sum_a\rho(s', a)$ will lie on the boundary. In other words, the above constraints give $\sum\nolimits_{a\in\mathcal{A}}\rho(s',a) = \sum\nolimits_{s,a}\Tilde{P}_e(s'|s, a)\rho(s, a)$. Further, we note that the region for the constraints is convex. This is because the set $\{x,y,z:xy\ge z\}$ is convex when $x, y, z \ge 0$. %Thus, the convex optimization problem can be efficiently solved. 
We note that even though the optimization problem may look non-convex due to constraints having product of two variables, we see Equations \eqref{eq:optimization_equation}, \eqref{eq:eps_cmdp_constraints}, and \eqref{eq:opt_eps_transition_constraint}-\eqref{eq:opt_transition_probability} form a convex optimization problem. We expand more on this in Appendix \ref{sec:convex_opt}. We note that \citep{rosenberg2019online} provide another approach to obtain a convex optimization problem for optimistic MDP. 

\input{ICML/algorithm_table}

% {\bf Mridul, explain 2nd equation - (24)}

Let $\rho_e$ be the solution for $\epsilon_e$-tight optimization equation for the optimistic MDP. Then, we obtain the optimal conservative policy for epoch $e$ as:
\begin{align}
    \pi_e(a|s) = \frac{\rho_e(s,a)}{\sum_{b\in\mathcal{A}}\rho_e(s,b)} \forall\ s,a \label{eq:opt_cons_optimal_policy}
\end{align}
The agent plays the optimistic conservative policy $\pi_e$ for  epoch $e$. Note that the conservative parameter $\epsilon_e$ decays with time. As the agent interacts with the environment, the system model improves and the agent does not need to be as conservative as before. This allows us to bound both constraint violations and the objective regret. Further, if during the initial iterations of the algorithms a conservative solution is not feasible, we can ignore the constraints completely. We will show that the conservation behavior is required when $t = \Theta(T)$ to compensate for the violations in the initial period of the algorithm \ref{sec:conservative_effect}.

For the \NAM\ algorithm described in Algorithm \ref{alg:algorithm}, we choose $\{\epsilon_e\} = \{K\sqrt{(\log t_e)/t_e}\}$. 
% The value of the Slater's constant $\delta$ must be at least $\epsilon_e \forall\ {e}$ to ensure that the constraints are satisfied. 
However, if the agent has access to a lower bound $T_l$ (Assumption \ref{slaters_conditon}) on the time horizon $T$, the algorithm can change the $\epsilon_e =K\sqrt{(\ln (t_e \vee T_{l}))/(t_e\vee T_{l})} \le \delta$ in each epoch $e$ as follows.
Note that if $T_l = 0$, $\epsilon_e$ becomes as specified in Algorithm \ref{alg:algorithm} and if $T_l = T$, $\epsilon_e$ becomes constant for all epochs $e$.

% {\bf Mridul, Since $\log t_e)/t_e$ decreases for $t_e>1$, does that not mean $\delta>1/2$ without knowledge on $T_l$ and  $\log T_l)/T_l$ - if so, say explicitly. Also, how to handle $t_e=1$ case?}




==> algorithm_table.tex <==
\begin{algorithm}[tb]
\caption{\NAM}
\label{alg:algorithm}
\textbf{Parameters}: $K$\\
\textbf{Input}: $S$, $A$, $r$, $d$, $c_i\ \forall\ i\in[d]$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $t=1$, $e = 1, \epsilon_e = K\sqrt{\frac{\ln t}{t}}$
\FOR{$(s,a) \in \mathcal{S}\times\mathcal{A}$}
    \STATE $\nu_e(s,a) = 0, N_e(s,a) = 0, \widehat{P}(s',a,s) = 0\forall\ s'\in\mathcal{S}$
\ENDFOR
\STATE Solve for policy $\pi_e$ using Eq. \eqref{eq:opt_cons_optimal_policy}
\FOR{$t \in \{1, 2, \cdots\}$}
    \STATE Observe $s_t$, and play $a_t\sim\pi_e(\cdot|s_t)$
    \STATE Observe $s_{t+1}$, $r(s_t,a_t)$ and $c_i(s_t, a_t)\ \forall\ i\in[d]$
    \STATE $\nu_e(s_t, a_t) = \nu_e(s_t, a_t) + 1$
    \STATE $\widehat{P}(s_t, a_t, s_{t+1}) = \widehat{P}(s_t, a_t, s_{t+1}) + 1$
    \IF {$\nu_e(s,a) = \max\{1, N_e(s,a)\}$ for any $s,a$}
        \FOR{$(s,a) \in \mathcal{S}\times\mathcal{A}$}
            \STATE $N_{e+1}(s,a) = N_e(s,a) + \nu_e(s,a)$
            \STATE $e = e+1$, $\nu_e(s,a) = 0$
        \ENDFOR
        \STATE $\epsilon_e = K\sqrt{\frac{\ln t}{t}}$
        \STATE Solve for policy $\pi_e$ using Eq. \eqref{eq:opt_cons_optimal_policy}
    \ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> figure_file.tex <==
\begin{figure*}[!t]
    \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=1\linewidth,trim={0.15in 0 0.6in 0.5in},clip]{model-regret.png}
         \caption{Regret decay \textit{w.r.t.} time}
         \label{fig:reward_regret}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=1\linewidth,trim={0.15in 0 0.6in 0.5in},clip]{model-service.png}
         \caption{Service constraints \textit{w.r.t.} time}
         \label{fig:service_const}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=1\linewidth,trim={0.15in 0 0.6in 0.5in},clip]{model-flow.png}
         \caption{Flow constraints \textit{w.r.t.} time}
         \label{fig:flow_const}
     \end{subfigure}    
    \caption{Performance of the proposed \NAM\ algorithm on a flow and service control problem for a single queue with respect to algorithmic parameter $K$ and choice of policy update times. The algorithm does not violate the constraints for higher value of $K$ at the expense of rewards regret.}
    \label{fig:Learning process}
    \vspace{-1.25em}
\end{figure*}


==> intro.tex <==
\section{Introduction}
% Reinforcement Learning is being increasingly applied to various interesting Markov Decision Processes (MDP) setups where the system model is not known apriori \cite{sutton2018reinforcement,recht2019tour}. Various algorithms have been developed to learn efficient policies using deep neural networks \cite{mnih2015human,schulman2017proximal,haarnoja2018soft}. Much work is also done to develop algorithms that are provably sample-efficient \cite{jaksch2010near,agrawal2017optimistic,jin2018provably}. However, 
In many applications where a learning agent uses reinforcement learning to find optimal policies, the agent optimizes a concave function of the expected rewards or must satisfy certain constraints while maximizing an objective \citep{altman1991constrained,roijers2013survey}. For example, in network scheduling, the controller may attempt to maximize fairness of the users using a concave function of the average rewards received by each of the users \citep{chen2021bringing}.
%a good policy for reaching a target pose should avoid hazardous poses which may damage the environment \cite{achiam2017constrained}. 
Or, consider autonomous vehicles where the goal is not just to reach the destination as early as possible, but also to ensure the safety of the surroundings \citep{le2019batch,tessler2018reward}. Further, there are certain environments in which the agent is required to ensure the constraint violations are reduced while optimizing the objective as well \citep{leike2017ai,ray2019benchmarking}. 

Recently, there has been significant effort to make RL algorithms for setups with constraints, or concave utilties, or both. For episodic setup, works range from model based algorithms \citep{brantley2020constrained,yu2021morl} to primal-dual based model-free algorithms \citep{ding2021provably}. Much recently, \citep{wei2021provably} proposed TripleQ algorithm which achieves zero constraint violations %\footnote{We note that even with zero constraint violations, an agent can violate constraints in the initial learning periods. Hence, zero constraints violations should be treated as $O(1/T)$, \textit{i.e.}, $O(1)$ violations in time $T$.} 
at the expense of an increased regret order of $O(K^{4/5})$ in episodic setup. However, for the episodic setup, the majority of the current work considers the weaker regret definition specified by \citep{efroni2020exploration}. Averaging constraint violations over multiple episodes allows constraint to oscillate around the boundary which implies that the policy (and the corresponding value function) may not converge to the optimal policy which satisfies the constraints.

The definition which considers the average over time makes sense for an infinite horizon setup as the long-term average is naturally defined \citep{puterman2014markov}. For a tabular infinite-horizon setup, \citep{singh2020learning} proposed an epoch-based algorithm which bounds the regret by $O(T^{2/3})$. Much recently, \citep{chen2022learning} proposed an Optimistic Online Mirror Descent based algorithm which obtains a regret bound of $O(T_M\sqrt{T})$ with $O(T_M^2S^3A)$ constraint violations for ergodic MDPs with $T_M$ mixing time.
We improve prior results on multiple fronts. First, we consider convex function for objectives and constraints. Second, even with a non-linear function setup, we reduce the regret order to $O(T_MS\sqrt{A/T})$ and bound the constraint violations with $0$. Finally, our algorithm does not require the knowledge of the time horizon $T$, whereas, the algorithms by \citep{singh2020learning,chen2022learning} requires the knowledge of $T$. %We compare our proposed algorithm with different related works in Table \ref{tab:algo_comparisons}.

In this work, we consider the problem of maximizing concave utility of the expected rewards while also ensuring that a set of convex constraints of the expected rewards are also satisfied. Moreover, we aim to develop algorithms that can also ensure that the constraints are not violated during the training phase as well. We work with tabular MDP with infinite horizon. For such setup, our algorithm updates policies  as it learns the system model. Further, our approach also bound the accumulated observed constraint violations as compared to the expected constraint violations.

To achieve this result, we propose an optimism based \NAM\ algorithm which proceeds in epochs $e$. At each epoch, we solve for an policy which considers constraints tighter by $\epsilon_e$ than the true bounds for the optimistic MDP in the confidence intervals for the transition probabilities. Further, as the knowledge of the model improves with increased interactions with the environment, we reduce this tightness. This $\epsilon_e$-sequence is critical to our algorithm as, if the sequence decays too fast, the constraints violations cannot be bounded by zero. And, if this sequences decays too slow, the objective regret may not decay fast enough. Further, using the $\epsilon_e$-sequence, we do not require the knowledge of the total time $T$ for which the algorithm runs.

We bound our regret by bounding the gap between the optimal policy in the feasible region and the optimal policy for the optimization problem with $\epsilon_e$ tight constraints. We bound this gap with a multiplicative factor of $O(1/\delta)$, where $\delta$ is Slater's parameter. Based on our analysis using the Slater's parameter $\delta$, we consider a case where a lower bound $T_l$ on the time horizon $T$ is known. This knowledge of $T_l$ allows us to relax our assumption on $\delta$. 

Further, for the regret analysis of the proposed \NAM\ algorithm, we use Bellman error for infinite horizon setup to bound the difference between the performance of optimistic policy on the optimistic MDP and the true MDP. Compared to analysis of \citep{jaksch2010near}, this allows us to work with stochastic policies. We bound our regret as $\Tilde{O}(\frac{1}{\delta}LdT_MS\sqrt{A/T} + CT_MS^2A/(1-\rho))$ and constraint violations as $0$, where $S$ and $A$ are the number of states and actions respectively, $L$ is the Lipschitz constant of the objective and constraint functions, $d$ is the number of costs the agent is trying to optimize, and $T_M$ is the mixing time of the MDP. The Bellman error based analysis along with Slater's slackness assumption also allows to develop posterior sampling based methods for constrained RL (see Appendix \ref{sec:psrl}) by showing feasibility of the optimization problem for the sampled MDPs.





==> regret.tex <==
\newpage
\section{Regret Analysis}
After describing \NAM\ algorithm, we now perform the regret and constraint violation analysis using Bellman error. We note that the standard analysis for infinite horizon tabular MDPs of UCRL2 \cite{jaksch2010near} cannot be directly applied as the policy $\pi_e$ is possibly stochastic for every epoch. Another peculiar aspect of the analysis of the infinite horizon MDPs is that the regret grows linearly with the number of epochs (or policy switches). This is because a new policy induces a new Markov chain and this chain  take time to converge to the stationary distribution. The analysis still bounds the regret by $\Tilde{O}(T_MS\sqrt{A/T})$ as the number of epochs are bounded by $O(SA\log T)$.
%We also note that the analysis of UCRL-CMDP \cite{singh2020learning} bounds the deviations with value function instead of bias resulting in regret scaling as $O(T^{-1/4})$.
% Compared to these works, our analysis works with stochastic policies, obtains regret independent to number of epochs, and scales as $\Tilde{O}(1/\sqrt{T})$. Hence, our analysis can be used as a tool to tightly analyze other learning algorithms for tabular infinite horizon MDPs. 

Before diving into the details, we first define few important variables which are key to our analysis. The first variable is the standard $Q$-value function. We define $Q_\gamma^{\pi, P}$ as the long term expected reward on taking action $a$ in state $s$ and then following policy $\pi$ for the MDP with transition $P$. Mathematically, we have
\begin{align}
Q_\gamma^{\pi, P}(s,a) = r(s,a) + \gamma\sum\nolimits_{s'\in\mathcal{S}}P(s'|s,a)V_\gamma^{\pi,P}(s').\nonumber
\end{align}
We also define Bellman error $B^{\pi, \Tilde{P}}(s,a)$ for the infinite horizon MDPs as the difference between the cumulative expected rewards obtained for deviating from the system model with transition $\Tilde{P}$ for one step by taking action $a$ in state $s$ and then following policy $\pi$. We have:
\begin{align}
    B^{\pi, \Tilde{P}}(s,a)&= \lim_{\gamma\to 1}\Big(Q_\gamma^{\pi, \Tilde{P}}(s,a) - r(s,a) -  \gamma\sum\nolimits_{s'\in\mathcal{S}}P(s'|s,a)V_\gamma^{\pi, \Tilde{P}}(s,a)\Big) \label{eq:Bellman_error_definition}
\end{align}
After defining the key variables, we can now jump into bounding the objective regret $R(T)$. Intuitively, the algorithm incurs regret on three accounts. First source is following the conservative policy which we require to limit the constraint violations. Second source of regret is solving for the policy which is optimal for the optimistic MDP. Third source of regret is the stochastic behavior of the system. We also note that the constraints are violated because of the imperfect MDP knowledge and the stochastic behavior. However, the conservative behavior actually allows us to violate the constraints within some limits which we will discuss in the later part of this section.

We start by stating our first lemma which relates the regret because we solve for a conservative policy. We define $\epsilon_e$-tight optimization problem as optimization problem for the true MDP with transitions $P$ with $\epsilon=\epsilon_e$. We bound the gap between the value of function $f$ at the long-term expected reward of the policy for $\epsilon_e$-tight optimization problem and the true optimization problem (Equation \eqref{eq:optimization_equation}-\eqref{eq:cmdp_constraints}) in the following lemma.

\begin{lemma}\label{lem:optimality_gap_objective}
Let $\lambda_{\pi^*}^P$ be the long-term average reward following the optimal feasible policy $\pi^*$ for the true MDP $\mathcal{M}$ and let $\lambda_{\pi_e}^P$ be the long-term average rewards following the optimal policy $\pi_e$ for the $\epsilon_e$ tight optimization problem for the true MDP $\mathcal{M}$, then for $\epsilon_e \le \delta$, we have,
\begin{align}
    &f\left(\lambda_{\pi^*}^P\right) -f\left(\lambda_{\pi_e}^P\right) \le 2L\epsilon_e/\delta
\end{align}
\end{lemma}
\begin{proof}[Proof Sketch]
We construct a policy for which the steady state distribution is the weighted average of two steady state distributions. First distribution is for the optimal policy for the true optimization problem. Second distribution is for the policy which satisfies Assumption \ref{slaters_conditon}. Now, we show that this constructed policy satisfies the $\epsilon_e$-tight constraints. Now, using Lipschitz continuity, we convert the difference between function values into the difference between the long-term average rewards to obtain the required result. The detailed proof is provided in Appendix \ref{app:proof_of_epsilon_gap_objective}.
\end{proof}

Lemma \ref{lem:optimality_gap_objective} and our construction of $\epsilon_e$ sequence allows us to limit the growth of regret because of conservative policy by $\Tilde{O}(LdT_MS\sqrt{A/T})$.

To bound the regret from the second source, we use a Bellman error based analysis. In our next lemma, we show that the difference between the performance of a policy on two different MDPs is bounded by long-term averaged Bellman error. Formally, we have:
\begin{lemma}\label{lem:bound_average_by_bellman_main}
The difference of long-term average rewards for running the optimistic policy $\pi_e$ on the optimistic MDP, $\lambda_{\pi_e}^{\Tilde{P}_e}$, and the average long-term average rewards for running the optimistic policy $\pi_e$ on the true MDP, $\lambda_{\pi_e}^P$, is the long-term average Bellman error as
\begin{align}
    \lambda_{\pi_e}^{\Tilde{P}_e} - \lambda_{\pi_e}^P = \sum\nolimits_{s,a}\rho_{\pi_e}^P B^{\pi_e, \Tilde{P}_e}(s,a)
\end{align}
\end{lemma}
\begin{proof}[Proof Sketch]
We start by writing $Q_\gamma^{\pi_e, \Tilde{P}_e}$ in terms of the Bellman error. Now, subtracting $V_\gamma^{\pi_e, P}$ from $V_\gamma^{\pi_e, \Tilde{P}_e}$ and using the fact that $\lambda_{\pi_e}^P = \lim_{\gamma\to1}V_\gamma^{\pi,P}$ and $\lambda_{\pi_e}^{\Tilde{P}_e} = \lim_{\gamma\to1}V_\gamma^{\pi,{\Tilde{P}_e}}$ we obtain the required result. A complete proof is provided in Appendix \ref{app:bounding_imperferct_model_regret}.
\end{proof}

After relating the gap between the long-term average rewards of policy $\pi_e$ on the two MDPs, we now want to bound the sum of Bellman error over an epoch. For this, we first bound the Bellman error for a particular state action pair $s,a$ in the form of following lemma. We have,
\begin{lemma}\label{lem:bound_bellman_s_a_main}
With probability at least $1- 1/t_e^6$, the Bellman error $B^{\pi_e, \Tilde{P}_e}(s,a)$ for state-action pair $s,a$ in epoch $e$ is upper bounded as
\begin{align}
B^{\pi_e, \Tilde{P}_e}(s,a) \le \sqrt{\frac{14S\log(2AT)}{1\vee N_e(s,a)}}\|\Tilde{h}\|_\infty
\end{align}
where $N_e(s,a)$ is the number of visitations to $s,a$ till epoch $e$ and $\Tilde{h}$ is the bias of the MDP with transition probability $\Tilde{P}_e$.
\end{lemma}
\begin{proof}[Proof Sketch]
We start by noting that the Bellman error essentially bounds the impact of the difference in value obtained because of the difference in transition probability to the immediate next state. We bound the difference in transition probability between the optimistic MDP and the true MDP using the result from \cite{weissman2003inequalities}. This approach gives the required result. A complete proof is provided in Appendix \ref{app:bounding_imperferct_model_regret}.
\end{proof}

We use Lemma \ref{lem:bound_average_by_bellman_main} and Lemma \ref{lem:bound_bellman_s_a_main} to bound the regret because of the imperfect knowledge of the system model. We bound the expected Bellman error in epoch $e$ starting from state $s_{t_e}$ and action $a_{t_e}$ by constructing a Martingale sequence with filtration $\mathcal{F}_t = \{s_1, a_1, \cdots, s_{t-1}, a_{t-1}\}$ and using Azuma's inequality \cite{bercu2015concentration}. Using the Azuma's inequality, we can also bound the deviations because of the stochasticity of the Markov Decision Process. The result is stated in the following lemma with proof in Appendix \ref{app:regret_bounds}.
\begin{lemma}
With probability at least $1-T^{-5/4}$, the regret incurred from imperfect model knowledge and process stochastics is bounded by
\begin{align}
    O(T_MS\sqrt{A(\log AT)/T} + (CT_MS^2A\log T)/(1-\rho))
\end{align}
\end{lemma}
The regret analysis framework also prepares us to bound the constraint violations as well. We again start by quantifying the reasons for constraint violations. The agent violates the constraint because \textbf{1.} it is playing with the imperfect knowledge of the MDP and \textbf{2.} the stochasticity of the MDP which results in the deviation from the average costs. We note that the conservative policy $\pi_e$ for every epoch does not violate the constraints, but instead allows the agent to manage the constraint violations because of the imperfect model knowledge and the system dynamics.

We note that the Lipschitz continuity of the constraint function $g$ allows us to convert the function of $d$ averaged costs to the sum of $d$ averaged costs. Further, we note that we can treat the cost similar to rewards \cite{brantley2020constrained}. This property allows us to bound the cost incurred incurred in a way similar to how we bound the gap from the optimal reward by $LdT_MS\sqrt{A(\log AT)/T}$. We now want that the slackness provided by the conservative policy should allow $LdT_MS\sqrt{A(\log AT)/T}$ constraint violations. This is ensured by our chosen $\epsilon_e$ sequence. We formally state that result in the following lemma proven in parts in Appendix \ref{app:regret_bounds} and Appendix \ref{app:constraint_violation_bounds}.
\begin{lemma}
The cumulative sum of the $\epsilon_e$ sequence is upper and lower bounded as,
\begin{align}
    \sum\nolimits_{e=1}^E(t_{e+1}-t_e)\epsilon_e = \Theta \left(K\sqrt{T\log T}\right)
\end{align}
\end{lemma}
After giving the details on bounds on the possible sources of regret and constraint violations, we can formally state the result in the form of following theorem.

\begin{theorem}\label{thm:regret_bound}
For all $T$ and $K = \Theta(LdT_MS\sqrt{A} + CSA/(1-\rho))$, the regret $R(T)$ of \NAM\ algorithm is bounded by 
\begin{align}
    R(T) = O\left(\frac{1}{\delta}LdT_MS\sqrt{A\frac{\log AT}{T}} + \frac{CT_MS^2A\log T}{1-\rho}\right)
\end{align}
and the constraints are bounded as $C(T) = 0$, with probability at least $1-\frac{1}{T^{5/4}}$.
\end{theorem}

\subsection{Posterior Sampling Algorithm} \label{sec:psrl_algorithm_main}
We can also modify the analysis to obtain Bayesian regret for a posterior sampling version of the UC-CURL algorithm using \cite[Lemma 1]{osband2013more}. In the posterior sampling algorithm, instead of finding the optimistic MDP, we sample the transition probability $\Tilde{P}_e$ using an updated posterior. This sampling allows to reduce the complexity of the optimization problem by eliminating Eq. \eqref{eq:boundary} and Eq. \eqref{eq:opt_transition_probability}. The complete algorithm is described in Appendix \ref{sec:psrl}. We note that optimization problem for the UC-CURL algorithm is feasible because the true MDP lies in the confidence interval. However, for the sampled MDP obtaining the feasibility requires a stronger Slater's condition. 

\subsection{Further Modifications} \label{sec:modifications}
The proposed algorithm, and the analysis can be easily extended to $M$ convex constraints $g_1, \cdots, g_M$ by applying union bounds. Further, our analysis uses \cite[Proposition 1]{jaksch2010near} to bound the epochs by $O(SA\log_2 T)$. However, we can improve the empirical performance of the \NAM\ algorithm by modifying the epoch trigger condition (Line 11 of Algorithm \ref{alg:algorithm}). Triggering a new episode whenever $\nu_e(s,a)$ becomes $\max\{1, \nu_{e-1}(s,a) + 1\}$ for any state-action pair results in a linearly increasing episode length with total epochs bounded by $O(SA + \sqrt{SAT})$. This modification results in a better empirical performance (See Appendix \ref{app:sim_details} for simulations) at the cost of a higher theoretical regret bound and computation complexity for obtaining a new policy at every epoch.



% Our Bellman error based analysis allows us remove the dependency on bounding the number of epochs for infinite-horizon MDPs algorithms. We believe this is an important step to possibly close the gap between the finite-horizon MDP algorithms infinite-horizon MDP algorithms. Further, our decaying conservative parameter $\epsilon_e$ also clears way to reduce dependency on parameter knowledge of $T$ for practical algorithms. 

% The agent solves for the $\epsilon_e$-tight optimization problem for the optimistic MDP at every epoch which may be a computationally inefficient step. %Thus, an agent can still prefer to choose a lesser number of epochs to reduce this computational cost. 
% Thus, an agent can choose a tradeoff between sample efficiency by updating policy frequently and computational efficiency of the logarithmic number of epochs.
% %We note that our algorithm requires the knowledge of $D$ for creating $\epsilon_e$ sequence, which may not be possible in some scenarios. We observe that choosing a large enough constant works well in practice as we will show in our next section.\\


==> related.tex <==
\section{Related Works}

% \textbf{Unconstrained RL:} %Stochastic Optimization using Markov Decision Processes has been studied extensively \citep{howard:dp,puterman2014markov,BertsekasTsitsiklis96}. For the unconstrained setup, initial works involved developing algorithms which can return optimal policies with the knowledge of underlying MDPs \cite{BertsekasTsitsiklis96}. \citep{Watkins1992} provided Q-learning based algorithm \cite{Watkins1992} which learn efficient policies without learning the transition model but by learning the effect of actions.
%IF Required, removed the previous paragraph.
% Much work has been done to understand finite time performance of algorithms for the tabular setup. \citep{jaksch2010near} provided epoch based UCRL2 algorithm which achieves a regret bound of $\Tilde{O}(DS\sqrt{A/T})$ for infinite horizon setup using optimism and proved a lower bound of $O(\sqrt{DSA/T}$ for MDPs with diameter $D$. \citep{fruit2018efficient} provided an improved epoch based SCAL algorithm with regret $O(D\sqrt{SA/T})$. The analysis of both UCRL2 and SCAL algorithm have an additional regret which increases linearly in the number of epochs. However, the algorithm bound the number of epochs in logarithmic order of time horizon $T$.   %For the episodic setup, recent works involve, optimism based provably efficient value iteration methods \cite{azar17UCBVI}, and Q-learning methods \cite{jin2018provably}.

\noindent\textbf{Constrained RL:} \citep{altman1999constrained} builds the formulation for constrained MDPs to study constrained reinforcement learning and provides algorithms for obtaining policies with known transition models. %Recently there is progress towards understanding the convergence properties and finite time performance of algorithms for unknown transition models. 
\citep{zheng2020constrained} considered an episodic CMDP and use an optimism based algorithm to bound the constraint violation as $\Tilde{O}(1/T^{0.25})$ with high probability. \citep{kalagarla2020sample} also considered the episodic setup to obtain PAC-style bound for an optimism based algorithm. \citep{ding2021provably} considered the setup of $H$-episode length episodic CMDPs with $d$-dimensional linear function approximation to bound the constraint violations as $\Tilde{O}(d\sqrt{H^5/T})$ by mixing the optimal policy with an exploration policy. \citep{efroni2020exploration} proposes a linear-programming and primal-dual policy optimization algorithm to bound the regret as $O(S\sqrt{H^3/T})$. \citep{wei2021provably, liu2021learning} considered the problem of ensuring zero constraint violations using a model-free algorithm for tabular MDPs with linear rewards and constraints. However, for infinite horizon setups, the analysis from finite horizon algorithms does not directly holds. This is because finite horizon setups can update the policy after every episode. But this policy switch modifies the induced Markov chains which takes time to converge to stationary distribution. 
% \citep{qiu2020cmdp} proposed an algorithm which obtains a regret bound of $\Tilde{O}(S\sqrt{AH^2/T})$ for the problem of adversarial stochastic shortest path. 
 
\citep{xu2020primal} consider an infinite horizon discounted setup with constraints and obtain global convergence using policy gradient algorithms. \citep{ding2020natural} also considers an infinite horizon discounted setup. They use a natural policy gradient to update the primal variable and sub-gradient descent to update the dual variable. \citep{singh2020learning} considered the setup of infinite-horizon ergodic CMDPs with long-term average constraints with an optimism based algorithm. \citep{gattami2021reinforcement} analyzed the asymptotic performance for Lagrangian based algorithms for infinite-horizon long-term average constraints, however they only show convergence guarantees without explicit convergence rates. \citep{chen2022learning} provide an optimistic online mirror descent algorithm for ergodic MDPs which obtain a regret bound of $O(T_MS\sqrt{SAT})$, and \citep{wei2022provably} provide a model free SARSA algorithm which obtains a regret bound of $O(\sqrt{SA}T^{5/6})$ for discounted constrained MDPs. \cite{liu2021fast} also an algorithm which achieves $\Tilde{O}(1/\epsilon^3)$ sample complexity to obtain zero constraint violations in infinite horizon discounted setup.
%We also consider ergodic CMDP similar to previous works but our setup also considers convex constraints and concave objectives. We propose optimism based algorithm to bound the regret as $\Tilde{O}(LdT_MS\sqrt{A/T})$ and posterior sampling based algorithm with $\Tilde{O}(LdT_MS\sqrt{A/T})$ Bayesian regret bound.

\input{ICML/related_table}

\noindent\textbf{Concave Utility RL:} Another major research area related to this work is concave utility RL \citep{hazan2019provably}. Along this direction, \citep{cheung2019regret} considered a concave function of expected per-step vector reward and developed an algorithm using Frank-Wolfe gradient of the concave function for tabular infinite horizon MDPs. \citep{agarwal2019reinforcement} also considered the same setup using a posterior sampling based algorithm. Recently, \citep{brantley2020constrained} combined concave utility reinforcement learning and constrained reinforcement learning for an episodic setup. \citep{yu2021morl} also considered the case of episodic setup with concave utility RL. However, both \citep{brantley2020constrained} and \citep{yu2021morl} consider the weaker regret definition by \citep{efroni2020exploration}, and \citep{cheung2019regret} and \citep{yu2021morl} do not target the convergence of the policy. Further, these works do not target zero-constraint violations.

Compared to prior works, we consider the constrained reinforcement learning with convex constraints and concave objective function. Using infinite-horizon setup, we consider the tightest possible regret definition. Further, we achieve zero constraint violations with objective regret tight in $T$ using an optimization problem with decaying tightness. A comparative survey of prior works and our work is also presented in Table \ref{tab:algo_comparisons}.


==> setup.tex <==
\section{Problem Formulation}\label{sec:system_model}

We consider an ergodic tabular infinite-horizon constrained Markov Decision Process $\mathcal{M} = (\mathcal{S}, \mathcal{A}, r, f, c_1, \cdots, c_d, g, P)$. $\mathcal{S}$ is finite set of $S$ states, and $\mathcal{A}$ is a finite set of $A$ actions. $P:\mathcal{S}\times\mathcal{A}\to\Delta(\mathcal{S})$ denotes the transition probability distribution such that on taking action $a\in\mathcal{A}$ in state $s\in\mathcal{S}$, the system moves to state $s'\in\mathcal{S}$ with probability $P(s'|s,a)$. $r:\mathcal{S}\times\mathcal{A}\to[0,1]$ and $c_i:\mathcal{S}\times\mathcal{A}\to[0,1], i\in{1, \cdots, d}$ denotes the average reward obtained and average costs incurred in state action pair $(s,a)\in \mathcal{S}\times\mathcal{A}$. 

The agent interacts with $\mathcal{M}$ in time-steps $t\in{1, 2, \cdots}$ for a total of $T$ time-steps. We note that $T$ is possibly unknown. At each time $t$, the agent observes state $s_t$, plays action $a_t$. The agent selects an action on observing the state $s$  using a policy $\pi:\mathcal{S}\to\Delta(\mathcal{A})$, where $\Delta(\mathcal{A})$ is the probability simplex on the action space. On following a policy $\pi$, the long-term average reward of the agent is denoted as:
\begin{align}
\lambda_{\pi}^P &= \lim_{\tau\to\infty}\mathbb{E}_{\pi,P}\left[\sum\nolimits_{t=1}^\tau r(s_t,a_t)/\tau\right]
\end{align}
where $\mathbb{E}_{\pi, P}[\cdot]$ denotes the expectation over the state and action trajectory generated from following $\pi$ on transitions $P$. The long-term average reward can also be represented as:
\begin{align}
    \lambda_{\pi}^P = \sum\nolimits_{s,a}\rho_{\pi}^P(s,a)r(s,a)&= \lim_{\gamma\to1}(1-\gamma)V_\gamma^{\pi, P}(s)\ \forall s\in\mathcal{S}\nonumber
\end{align}
where $V_\gamma^{\pi, P}(s)$ is the discounted cumulative reward on following policy $\pi$, and $\rho_{\pi}^{P}\in\Delta(\mathcal{S}\times\mathcal{A})$ is the steady-state occupancy measure generated from following policy $\pi$ on MDP with transitions $P$ \cite{puterman2014markov}. Similarly, we also define the long-term average costs as follows:
\begin{align}
    \zeta_{\pi}^P(i) &= \lim_{\tau\to\infty}\mathbb{E}_{\pi,P}\left[\sum\nolimits_{t=1}^\tau c_i(s_t,a_t)/\tau\right] = \lim_{\gamma\to1}(1-\gamma)V_\gamma^{\pi, P}(s;i)\ \ \ \forall s\in\mathcal{S}\nonumber\\
    &= \sum\nolimits_{s,a}\rho_{\pi}^P(s,a)c_i(s,a)
\end{align}
The agent interacting with the CMDP $\mathcal{M}$ aims to maximize a function $f:[0,1]\to\mathbb{R}$ of the average per-step reward. Further, the agent attempts to ensure that a function of average per-step costs $g:[0,1]^d\to\mathbb{R}$ is at most $0$. 
The goal is represented mathematically as:
\begin{align}
    &\max_\pi f\left(\lambda_\pi^P\right)~~~s.t.~~~g\left(\zeta_{\pi}^P(1), \cdots, \zeta_{\pi}^P(d)\right) \le 0,
\end{align}

Let $P^{t}_{\pi, s}$ denote the $t$-step transition probability on following policy $\pi$ in MDP $\mathcal{M}$ starting from some state $s$. Also, let $T_{s\to s'}^\pi$ denotes the time taken by the Markov chain induced by the policy $\pi$ to hit state $s'$ starting from state $s$. Then let $T_M = T_M := \max_\pi \mathbb{E}[T^\pi_{s\to s'}]$ be the mixing time of the MDP $\mathcal{M}$. We now introduce our assumptions on the MDP $\mathcal{M}$.

\begin{assumption}\label{ergodic_assumption}
The MDP $\mathcal{M}$ is ergodic, or $\|P^t_{\pi, s} - P_{\pi}\| \le C\rho^t$ with $P_\pi$ being the long-term steady state distribution induced by policy $\pi$, and $C > 0$ and $\rho < 1$ are problem specific constants. And, the mixing time of the MDP $\mathcal{M}$ if finite or $T_M < \infty$.
\end{assumption}

\begin{assumption} \label{known_rewards}
The rewards $r(s,a)$, the costs $c_i(s,a); \forall \ i$ and the functions $f$ and $g$ are known to the agent.
\end{assumption}

\begin{assumption}\label{concave_assumption}
The scalarization function $f$ is jointly concave and the constraints $g$ are jointly convex. Hence for any arbitrary distributions $\mathcal{D}_1$ and $\mathcal{D}_2$, the following holds.
\begin{align}
    f\left(\mathbb{E}_{x\sim\mathcal{D}_1}\left[x\right]\right) &\geq \mathbb{E}_{x\sim\mathcal{D}_1}\left[f\left(x\right)\right]\label{eq:concave_utility}\\
    g\left(\mathbb{E}_{\mathbf{x}\sim\mathcal{D}_2}\left[\mathbf{x}\right]\right) &\leq \mathbb{E}_{\mathbf{x}\sim\mathcal{D}_2}\left[g\left(\mathbf{x}\right)\right];\ \mathbf{x}\in\mathbb{R}^d\label{eq:convex_constraints}
\end{align}
\end{assumption}

\begin{assumption}\label{lipschitz_assumption}
The function $f$ and $g$ are assumed to be a $L-$ Lipschitz function, or
    \begin{align}
        \left|f\left(x\right) - f\left(y\right)\right| &\leq L|x - y|;\ x,y\in\mathbb{R} \label{eq:Lipschitz}\\
        \left|g\left(\mathbf{x}\right) - g\left(\mathbf{y}\right)\right| &\leq L\left\lVert \mathbf{x} - \mathbf{y}\right\rVert_1;\ \mathbf{x}, \mathbf{y}\in\mathbb{R}^d \label{eq:cost_Lipschitz}
    \end{align}
\end{assumption}

\begin{remark}
We consider a standard setup of concave and the Lipschitz function as considered by \citep{cheung2019regret,brantley2020constrained,yu2021morl}. Note that the  analysis in this paper directly works for $f:\mathbb{R}^K\to\mathbb{R}$, where the function takes as input $K$ average per-step rewards for $K$ objectives. 
We can obtain maximum entropy exploration if choose function $f = -\sum_{k}\lambda_k\log(\lambda_k+\eta)$ with $r_k(s,a) = \bm{1}_{\{s_k, a_k\}}$ for a particular state action pair $s_k, a_k$ and choosing $K = S\times A$ to cover all state-action pairs and a regularizer $\eta$.
\end{remark}

\begin{assumption} \label{slaters_conditon}
There exists a policy $\pi$, and one constant $\delta > LdST_M\sqrt{(A\log T)/T} + (CSA\log T)/(T(1-\rho))$ such that 
\begin{align}
    g\left(\zeta_{\pi}^P(1), \cdots, \zeta_{\pi}^P(d)\right) \le -\delta
\end{align}
\end{assumption}
% Further, if there is a (possibly unknown) lower bound on time-horizon, $T_l\ge\exp{(1)}$, then we only require $\delta > LdST_M\sqrt{A(\log T_l)/T_l}$. 
This assumption is again a standard assumption in the constrained RL literature \citep{efroni2020exploration,ding2021provably,ding2020natural,wei2021provably}. $\delta$ is referred as Slater's constant. \citep{ding2021provably} assumes that the Slater's constant $\delta$ is known. \citep{wei2021provably} assumes that the number of iterations of the algorithm is at least $ \Tilde{\Omega}(SAH/\delta)^5$ for episode length $H$. On the contrary, we simply assume the existence of $\delta$ and a lower bound on the value of $\delta$ which gets relaxed as the agent acquires more time to interact with the environment.

Any online algorithm starting with no prior knowledge will require to obtain estimates of transition probabilities $P$ and obtain reward $r$ and costs $c_k, \forall\ k\in\{1,\cdots,d\}$ for each state action pair. Initially, when algorithm does not have good estimate of the model, it accumulates a regret as well as violates constraints as it does not know the  optimal policy.  We define reward regret $R(T)$ as the difference between the average cumulative reward obtained vs the expected rewards from running the optimal policy $\pi^*$ for $T$ steps, or
\begin{align}
    R(T)& = f\left(\lambda_{\pi^*}^P\right) - f\left(\sum\nolimits_{t=1}^Tr(s_t, a_t)/T\right) \nonumber%\label{eq:regret_rewards}
\end{align}
Additionally, we define constraint regret $C(T)$ as the gap between the constraint function and incurred and constraint bounds, or
\begin{align}
    C(T)& = \left(g\left(\sum\nolimits_{t=1}^Tc_1(s_t, a_t)/T, \cdots, \sum\nolimits_{t=1}^Tc_1(s_t, a_t)/T\right)\right)_+ \nonumber% \label{eq:regret_costs}.
\end{align}
where $(x)_+ = \max(0, x)$.

% {\bf Big issue in the definition and discussions. The regret as defined here is averaged and thus will be $1/\sqrt{T}$, while the intro etc. says $\sqrt{T}$. The constraint violation is also averaged, so $O(1)$ is obvious - woudn't $O(1/T)$ similiarly is what we prove? The key theorem also uses this C, so unclear - please be consistent in this. }

In the following section, we present a model-based algorithm to obtain this policy $\pi^*$, and reward regret and the constraint regret accumulated by the algorithm.






==> simulations.tex <==
\section{Experimental Studies}
\input{ICML/figure_file}
We now evaluate the empirical performance of the proposed \NAM\ algorithm using the flow and service control in a single-server queue, which is introduced in \citep{altman1991constrained}. 


We consider a discrete-time queue with a buffer of finite size $L$. The state is the number of customers waiting in the queue with $S = L+1$. The system has two types of actions, service and flow, to control the number of customers. At time $t$, the agent takes action $a_t = (a_t(1), a_t(2))$ from a finite subset of $[0,1]\times[0,1]$, where $a_t(1)$ is the service action and $a_t(2)$ is the flow action. The service action $a_t(1)$ reduces the queue length by $1$ with probability $a_t(1)$, and the flow action increases the queue by $1$ with probability $a_t(2)$. Also, we assume that there is no customer arriving when the queue is full. The precise environment and implementation details are provided in Appendix \ref{app:sim_details}.

For $a_t \sim \pi$, the optimization problem is defined as
\begin{align}
        \max_{\pi} &\quad \lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum\nolimits_{t=1}^{T}(5-s_t)\nonumber\\
        s.t. &\quad \lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum\nolimits_{t=1}^{T}(6-10a_t(1))\geq 0\nonumber\\
        &\quad \lim\limits_{T\rightarrow\infty}\frac{1}{T}\sum\nolimits_{t=1}^{T}(2-8(1-a_t(2))^2)\geq 0\nonumber
\end{align}
We use the length of horizon $T=10^5$ and run 100 independent simulations of the proposed \NAM\ algorithm. The result is shown in  Figure \ref{fig:Learning process}. The average values of the long-term averaged reward and the constraint functions are shown in the solid lines, and the shadow region denotes the standard deviation. In order to compare this result to the optimal, we assume that the full information of the transition dynamics is known and then use Linear Programming to solve the problem. The optimal expected reward from LP is $4.08$ for the true MDP. We now make the following observations based on the simulation results. 

\textbf{Effect of the frequency of policy updates}: We compare the \NAM\  algorithm in Algorithm \ref{alg:algorithm} with a modified algorithm which updates the policy after every interaction with the environment. The number of epochs in Algorithm \ref{alg:algorithm} is bounded by $O(SA\log(T))$ \cite{jaksch2010near} whereas the number of epochs of the modified algorithm is $T$. Our claim that the proposed regret bounds does not depend on the number epochs, is empirically evident in Figure \ref{fig:reward_regret}. The objective regret of the doubling epoch based algorithm \ref{alg:algorithm} matches the regret guarantees but does not outperform the empirical performance of the everytime policy update strategy. However, the doubling epoch based algorithm obtains lower constraint violations as the agent plays $\epsilon_e$- conservative policy for longer duration, thus violating constraints less (Figure \ref{fig:flow_const} and Figure \ref{fig:service_const}). The agent which updates the policy after every interaction, plays a lesser conservative policy resulting in empirically increased constraints violations, while achieving better regret empirically. 

\textbf{Effect of the parameter $K$ in \NAM\ algorithm}: We note that in practice the optimal $K= LdT_MS\sqrt{A}$ may be difficult to precisely calculate. Hence, we evaluate the proposed \NAM\ algorithm for various values of $K$. If we choose the multiplication factor $K=0$, we will not be achieving zero constraint violations but can still bound the constraint violations with $\Tilde{O}(LdT_MS\sqrt{A/T})$. Note that as we increase the value of $K$, the constraint violations decrease in Figure \ref{fig:service_const} and Figure \ref{fig:flow_const}. However, this results in a lower reward value as observed in Figure \ref{fig:reward_regret}. In principle, the agent must select $K$ which allows to obtain a feasible policy and reduce the violations.


%An advantage of the doubling epoch updates, however, is low computational cost.


